"Going on a vacation" takes longer than "Going for a walk": A Study of Temporal Commonsense Understanding

Understanding time is crucial for understanding events expressed in natural language. Because people rarely say the obvious, it is often necessary to have commonsense knowledge about various temporal aspects of events, such as duration, frequency, and temporal order. However, this important problem has so far received limited attention. This paper systematically studies this temporal commonsense problem. Specifically, we define five classes of temporal commonsense, and use crowdsourcing to develop a new dataset, MCTACO, that serves as a test set for this task. We find that the best current methods used on MCTACO are still far behind human performance, by about 20%, and discuss several directions for improvement. We hope that the new dataset and our study here can foster more future research on this topic.

==> intro_old_comment.tex <==


\ignore{
Due to the reporting bias that people usually do not say the obvious \cite{GordonVa13}, it is crucial for a computer to acquire commonsense knowledge and incorporate it into its decision making process \cite{forbes2017verb,ZRDV17,yang2018extracting,RSASC18,BauerWaBa18,TDGYBC18,zellers2018swag}.
}


% old version
\ignore{
In this work, we examine the existing systems in their ability to handle \emph{temporal commonsense} or such world knowledge. 
% In particular, we focus on \emph{temporal} aspects of commonsense understanding. 
In particular, we consider five temporal properties: \emph{duration} (typical event duration), \emph{stationarity} (whether an event lasts long-enough), \emph{temporal ordering} (typical order of events), \emph{typical time} (when do events usually happen), and \emph{frequency} (\qiang{how often an event occurs}). Our goal is to study how existing methods could understand all these attributes.
}

% difference with the typical time. 
\ignore{
The temporal problems we are interested here are different from what has been investigated in the field. 
While there are many works on understanding \emph{time}, a vast majority of efforts focus on problems that mostly involve semi-direct mentions in text: 
for instance, extraction and normalization of \emph{temporal mentions}, \emph{events}, and \emph{relations}, %etc.~
% "such as" cannot be followed by "etc."
\cite{strotgen2010heideltime,chang2012sutime,ning2017structured}. 
% This problem has been addressed in different levels, such as the extraction of \emph{temporal mentions}, \emph{events}, and \emph{relations}, %etc.~
% "such as" cannot be followed by "etc."
% \cite{strotgen2010heideltime,chang2012sutime,ning2017structured}.
However, many instances we consider here contains involve a  variety of temporal phenomena that appear implicitly, without direct temporal references. 
% (hence, temporal commonsense). 
% This implicit understanding is usually referred to as \emph{commonsense} understanding, as it is widely known by many people and rarely get direct mentions in text.
\qiangcomment{I feel that this discussion is not in the right position.}
}

\ignore{
\qiangcomment{please put refs for ESIM and BERT}.
}

\ignore{
\qiang{\sout{More details about \datasetname{} are in Sec.~\ref{sec:tacoqa}.}}
}

% old version
\ignore{
To have a natural evaluation to such properties, this paper introduces \datasetname, \textbf{t}empor\textbf{a}l \textbf{co}mmon-sense \textbf{q}uestion \textbf{a}nswering dataset, to serve as a diagnostic environment for further investigations dedicated to temporal commonsense. 
Our dataset is constructed with three meticulously-designed crowdsoursing stages. 
Figure~\ref{fig:intro:example} shows some examples for each class in \datasetname. 
The input contains a \emph{sentence} providing context information, a \emph{question} asking for temporal information, and \emph{candidate answers} with or without the correct ones in it.
To ensure the answers requires commonsense, no questions can be answered with a phrase explicitly contained in the context. 
% Note that we intentionally require that the answers to those questions should not be mentioned explicitly in the sentence, but humans can still infer them.
Moreover, we made sure that the question can still be answered with high agreement by human.
For example, \emph{Q1} asks whether that Mark is still on the farm. Given somebody being at some place's transient property, in addition to Mark is now a judge, humans can agree that he is no longer on the farm, even though the answer is not explicitly mentioned in \emph{S1}.
Similarly, \emph{Q5} asks for the frequency of large mammals' rest, and humans know that they usually rest every day, not too frequent (``once a minute'') or too infrequent (``once every three days'').
\qiangcomment{I feel that this paragraph can be shortened. It's too detailed right now.}
}


\begin{comment}
\daniel{OLD: 
Understanding \emph{time} and reasoning with it is crucial for many natural language 
% understanding 
tasks. This problem has been addressed in different levels, such as the extraction of \emph{temporal mentions}, \emph{events}, and \emph{relations}, %etc.~
% "such as" cannot be followed by "etc."
\cite{strotgen2010heideltime,chang2012sutime,ning2017structured}. 
However, a wide variety of temporal phenomena appear implicitly, without direct temporal references. This implicit understanding is usually referred to as \emph{commonsense} understanding, as it is widely known by many people and rarely get direct mentions in text. % For instance,
% The easiest problems for humans are usually the hardest for computers. Such problems often go unmentioned,
% due to their triviality (for humans). 
For instance, humans trivially know that there are many differences between ``going to college'' and ``going to the movies'' (e.g., duration and prerequisites)
%, etc). 
% again, "e.g.," cannot be followed by "etc."
% Our current technologies so far don’t have any responses to such problems.
% Solving high-level natural language end-tasks, such as dialogue, machine comprehension, textual entailment, requires an extensive use of \emph{commonsense} knowledge and reasoning~\cite{}. 
}



commonsense has been an active topic in NLP due to its importance for reasoning, but the acquisition of commonsense is challenging because it is rarely explicitly mentioned in text. 
\ben{I think rarely mentioned in text is inaccurate \qiangcomment{agreed; I think we can simply delete the discourse of "but"} (e.g, we can use ``for" pattern to collect huge amounts of knowledge on duration). I believe the real difficulty here is that there will never be enough supervision on this, and learning from unsupervised objectives are noisy, thus the representations are not ideal. }
Much attention has been paid to this area over the years, including open concepts \cite{HavasiSpAl07}, sentiments \cite{CambriaOlRa14},  adjective intensities \cite{CWPAC18}, and physical properties of actions and objects \cite{forbes2017verb,yang2018extracting}.
\qiangcomment{add more references.}

The capability of understanding and reasoning over {\em time} is crucial for many tasks, such as timeline construction \qiang{(refs)}, summarization \qiangcomment{don't know the refs here}, and causality inference \qiang{(refs)}, for which commonsense is also very important. 
\todo{
``concrete examples of upstream tasks that make use
  of systems that tackle the task/dataset in this paper.'' + 
  ``a more crisp connection between the task/dataset and these
  would make things more concrete.''
}
For example, to answer, {\em did Aristotle have a laptop?} one needs to at least reason about when Aristotle lived, when laptop was invented, and a person who had died could not have a laptop. 
However, such cases have hardly been studied.
\ben{I think we should change the example. \qiangcomment{agreed} Dead person cannot have new things is not strictly an aspect that we care in this work. What about one of our extended questions in Appendix A.2?}

\todo{Better (formal?) definition of the categories, somewhere near here?}
\todo{Related: ``define the scope of the task''}

To fill this gap, this paper introduces \datasetname, short for \textbf{t}empor\textbf{a}l \textbf{co}mmonsense \textbf{q}uestion \textbf{a}nswering dataset, to serve as a benchmark for further investigations dedicated to temporal commonsense.
% \todo{``the definition of the temporal aspects (we can appeal to the Hovy paper)'',}
Specifically, for the first time, we systematically categorize the phenomena in temporal commonsense into five classes: \emph{duration,  stationarity, temporal ordering, typical time, and frequency}.
\ben{Yes, I think we can include here some bullet points for definitions. Alternatively we can have a section just for temporal commonsense?}
Figure~\ref{fig:intro:example} shows some examples for each class in \datasetname. 
The input contains a \emph{sentence} providing context information, a \emph{question} asking for temporal information, and \emph{candidate answers} with or without the correct ones in it.
\ben{To ensure the answers requires commonsense, no questions can be answered with a phrase contained in the context. Moreover, we made sure that the question can still be answered with high agreement by human.}
Note that we intentionally require that the answers to those questions should not be mentioned explicitly in the sentence, but humans can still infer them.
For example, \emph{Q1} asks whether that ``she is known as Fontaine'' still holds true at a later time (i.e., a {\em transient} state or a {\em stationary} fact).
Although the answer is not explicitly mentioned in \emph{S1}, most humans can tell that a person does not change his/her name if not stated otherwise.
Similarly, \emph{Q5} asks for the frequency of people making trips, and humans know it is unlikely to happen every night.
\ben{I think we should select better examples, and provide better explanations.}
\ben{In addition, we do not provide training data for this dataset, only a small dev set that provides the definition of the task. This is because the test set heavily evaluates system's ability to acquire commonsense knowledge, so that end-to-end training makes no sense, as there will never be enough direct supervision. We expect a system to be capable of acquiring temporal commonsense from other sources (e.g. pre-training), then use the dev data to derive a reasoning/QA model. }
% about duration of a ``laughing'' event described in \emph{S3}. Any human knows that ``laughter'' usually last less than a few minutes or seconds (and not ``20 minutes'').

\todo{
This might be a good place to defend this criticism: 
``Has the author tried any time/number recognizing and normalization preprocessing (for sentences / questions / answers)?''
}
\end{comment}

\ignore{
\textbf{The contributions of this work can be summarized as follows.}\qiangcomment{I'm going to move the bullets below to different places in-text. Will work on it in the afternoon.}
\begin{itemize}[noitemsep,leftmargin=0.4cm]
    \item A high-quality dataset on \emph{temporal commonsense}, \datasetname, is collected via crowdsourcing, which can significantly facilitate further research along this direction.\footnote{The dataset and codes will be released upon publication.}
    \ignore{To facilitate this research towards the problem of \emph{temporal commonsense}, we create a high-quality dataset for this task using crowdsourcing.}
    
    \item Multiple systems based on the state-of-the-art (including \emph{ESIM} and \bert) are proposed and evaluated on \datasetname. 
    % , showing the current state-of-the-art on this problem.
    \ignore{We  develop
    % \ben{can we say create here?}
    multiple competitive systems using state-of-the-art machinery available in the field. Additionally we show that humans are able to achieve significantly higher score on this task. }
    
    \item We show that there remains a significant performance gap between the proposed systems and humans, indicating the limitations of current NLP techniques and pointing out potential research directions.
    \ignore{We provide extra analysis on limitations of current techniques and remaining open challenges.} 
    % We create competitive systems for each sub-task, using state-of-the-art techniques. 
    % We observe that complexity of the datset to machine solvers, 
    % for our dataset and show its complexity, 
    % as indicated by the performance gap with human.
    
\end{itemize}
}



% \daniel{ 
% OLD: 
% In this work we introduce \datasetname, a \underline{t}empor\underline{a}l \underline{co}mmon-sense \underline{q}uestion \underline{a}nswering dataset. The goal of this dataset is to provide a natural language testbed, 
% % in order 
% to measure the progress towards acquiring and applying \emph{temporal commonsense}. Figure~\ref{fig:intro:example} provides a few examples questions from our dataset. The inputs include a \emph{sentence} describing a situation, a \emph{temporal question} and collection of \emph{candidate answers}. None of the questions have explicit answers in the sentence; instead, their answers need to be 
% % have to 
% be \emph{inferred} from the given input. For example, \emph{Q1} is asking about the age of a ``structure'' described in \emph{S1}. While there is no direction mention of the answer in \emph{S1}, many humans are able guess how many years can a ``structure'' age and answer this question. Similarly, \emph{Q3} is asking about duration of a ``laughing'' event described in \emph{S3}. Any human knows that ``laughter'' usually last less than a few minutes or seconds (and not ``20 minutes''). 
% }


% To facilitate further analysis, each question comes with its reasoning category, such as \emph{event frequency, event duration, etc}. 
% A few sampled questions in our dataset are depicted in Figure~\ref{fig:intro:example}. For example, 
% A system, in order to answer such questions, it has to be equipped with the 

% sciene exams 
% textual entailment 
% The importance of real-world knowledge for natural language understanding has been well-understood. 
% For example, Winograd's
% Representing knowledge and automating reasoning about times, durations, and
% time intervals is a largely solved problem.
% For instance, if one knows that Mozart was born earlier and died younger than Beethoven, one can infer that Mozart died earlier than Beethoven. 
% If one knows the Battle of Trenton occurred during the Revolutionary War, the Battle of Gettysburg occurred during the Civil War, and the Revolutionary War was over before the Civil War started, then one can infer the Battle of Trenton occurred before the Battle of Gettysburg. The inferences involved here in almost all cases reduce to solving
% systems of linear inequalities, usually small and of a very simple form. Integrating such reasoning with specific applications, such as natural language interpretation, has been much more problematic. Natural language expressions for time are com

% \qiangcomment{I think we need to discuss the following things in intro: (1) Why is temporal common sense important? (2) How to formally define temporal common sense? (3) What are (and how do we position) our contributions? I feel that we did not do well in address all the three points.}



==> related_old.tex <==
\begin{comment}
\daniel{
OLD: 
Temporal information and inference is an important component in natural language understanding. There are multiple popular tasks related to temporal inference, such as temporal relation \cite{ning2018joint} and script generation \cite{leeuwenberg2018temporal} \cite{granroth2016happens}. These works have shown that temporal reasoning is essential yet challenging, as human performances are still much better than state-of-the-art systems across multiple benchmarks.
}

\daniel{
OLD: 
commonsense understanding has a long history as a critical part of machine reasoning as well, for both vision \cite{lin2015don} and NLP communities. Early work to address commonsense in languages are mostly focusing on acquiring commonsense information. \cite{liu2004conceptnet} proposed a large knowledge base of commonsense relations between entities. \cite{forbes2017verb} proposed a way to generate large scale commonsense knowledge of physical properties. \cite{williams2012extracting} proposed an early work on acquiring large-scale temporal duration information. With the acquired information, there has been recent successes in applying commonsense information for downstream tasks. \cite{yang2018extracting} proposed a model to learn physical relationships among properties, \cite{ning2018joint} ...
}

\daniel{
OLD: 
If we want to evaluate systems' abilities of acquiring and reasoning with commonsenses, it is natural to use question answering as the end task. People have done a lot in terms of gathering QA datasets as machine reading comprehension benchmarks. Most existing QA datasets for reading comprehension require the answer to have direct supporting evidences in the provided text, such as \cite{Richardson2013MCTestAC} and \cite{MultiRC2018}. We have seen more datasets that address the use of commonsense, in which the answers are not directly supported by the evidence. \cite{zellers2018swag} proposed a work of ending completion.
}
\end{comment}

\begin{comment}
commonsense understanding has a long history as a critical part of machine reasoning as well, for both vision \cite{lin2015don} and NLP communities. Early work to address commonsense in languages are mostly focusing on acquiring commonsense information. \cite{liu2004conceptnet} proposed a large knowledge base of commonsense relations between entities. \cite{forbes2017verb} proposed a way to generate large scale commonsense knowledge of physical properties. \cite{williams2012extracting} proposed an early work on acquiring large-scale temporal duration information. With the acquired information, there has been recent successes in applying commonsense information for downstream tasks. \cite{yang2018extracting} proposed a model to learn physical relationships among properties, \cite{ning2018joint} ...
\end{comment}
